Little Magnetic Book

This book is devoted to the spectral analysis of the magnetic Laplacian in various geometric situations. In particular the influence of the geometry on the discrete spectrum is analysed in many asymptotic regimes.

==> chapter-brokenwg.tex <==
\chapter{Spectrum of broken waveguides}\label{chapter-brokenwg}
\begin{flushright}
\begin{minipage}{0.65\textwidth}
In spite of all this, however, he did not lose sight of his raft, but swam as fast as he could towards it, got hold of it, and climbed on board again so as to escape drowning.
\begin{flushright} 
\textit{Odyssey}, Book V, Homer
\end{flushright}
\vspace*{0.5cm}
\end{minipage}
\end{flushright}
 
In this chapter we present the main ingredients in the proof of the two terms asymptotics in Theorem \ref{spectrum-guide}.

\section{Quasimodes}
As usual we shall introduce appropriate quasimodes. As we will see, we will have to introduce the notion of Dirichlet-to-Neumann operators to analyze the transmission between the corner and the \enquote{guiding part} of the waveguide.
\subsection{Preliminaries}
In order to construct quasimodes for $\mathcal{L}_{\Gui}(h)$ of the form $(\gamma_h,\psi_h)$, we use the coordinates $(u,t)$ on the left and $(u,\tau)$ on the right and look for quasimodes $\hat\psi_h(u,t,\tau)=\psi_h(x,y)$.
Such quasimodes will have the form on the left:
\begin{equation}
\label{6Alef}
   \psi_{\lef}(u,t) \sim \sum_{j\geq 0}h^{j/3}
   \left(\Psi_{\lef,j}(h^{-2/3}u,t)+ \Phi_{\lef,j}(h^{-1}u,t)\right),
\end{equation}
and on the right:
\begin{equation}
\label{6Ari}
   \psi_{\ri}(u,\tau)\sim\sum_{j\geq 0} h^{j/3} \Phi_{\ri,j}(h^{-1}u,\tau)
\end{equation}
associated with quasi-eigenvalues:
$$\gamma_h\sim\sum_{j\geq 0}\gamma_{j} h^{j/3}\,.$$
We will denote $s=h^{-2/3}u$ and $\sigma=h^{-1}u$.
Since $\psi_h$ has no jump across the line $x=0$, we find that $\psi_{\lef}$ and $\psi_{\ri}$ should satisfy two transmission conditions on the line $u=0$:
\begin{equation}\label{tramsission-cond}
   \psi_{\lef}(0,t)=\psi_{\ri}(0,t)
   \quad\mbox{and}\quad
   \left(\dr_{u}-\frac{t}{\pi\sqrt{2}}\dr_{t}\right)\psi_{\lef}(0,t) = 
   \left(\partial_u-\frac{\partial_\tau}{\pi\sqrt2}\right)\psi_{\ri}(0,t)\,,
\end{equation}
for all $t\in(0,1)$.
For the Ans\"atze \eqref{6Alef}-\eqref{6Ari} these conditions write for all $j\ge0$
\begin{align}
\label{transD}
  & \Psi_{\lef,j}(0,t)+\Phi_{\lef,j}(0,t)=\Phi_{\ri,j}(0,t) \\
\label{trans}
  & \dr_{\sigma}\Phi_{\lef,j}(0,t)+\dr_{s}\Psi_{\lef,j-1}(0,t)
   -\frac{t\dr_{t}}{\pi\sqrt{2}}\Phi_{\lef,j-3}(0,t)-\frac{t\dr_{t}}{\pi\sqrt{2}}\Psi_{\lef,j-3}(0,t)
  \\ \nonumber 
  & \hskip 18em =\dr_{\sigma}\Phi_{\ri,j}(0,t)
   -\frac{\partial_\tau}{\pi\sqrt2}\Phi_{\ri,j-3}(0,t)\,,
\end{align}
where we understand that the terms associated with a negative index are $0$.

\begin{notation}
\label{6not}
We still set $s=h^{-2/3}u$ and $\sigma=h^{-1}u$.
Like in the case of the triangle $\Tri$, the operators $\mathcal{L}^\lef_\Gui$ and $\mathcal{L}^\ri_\Gui$, written in variables $(s,t)$ and $(\sigma,t)$ expand in powers of $h^{2/3}$ and $h$, respectively. Now we have three operator series:
\begin{enumerate}[(i)]
\item $\mathcal{L}^\lef_\Gui(h)(h^{2/3}s,t;h^{-2/3}\partial_s,\partial_t) 
   \sim \sum_{j\geq 0} \mathcal{L}_{2j}h^{2j/3}$. The operators are the same as for $\Tri$, but they are defined now on the half-strip $\Stlef:=(-\infty,0)\times(0,1)$.

\item $\mathcal{L}^\lef_\Gui(h)(h\sigma,t;h^{-1}\partial_\sigma,\partial_t) \sim
   \sum_{j\geq 0} \mathcal{N}^\lef_{3j}h^{j}$ defined on $\Stlef$. 

\item $\mathcal{L}^\ri_{\Gui}(h)(h\sigma,\tau;h^{-1}\partial_\sigma,\partial_\tau) \sim
   \sum_{j\geq 0} \mathcal{N}^\ri_{3j}h^{j}$ defined on $\Stri:=(0,\infty)\times(0,1)$. 
\end{enumerate}
The boundary conditions of the operators $\mathcal{L}_j$, $\mathcal{N}^\lef_{j}$, and $\mathcal{N}^\ri_{j}$ are
\begin{enumerate}[(i)]
\item Neumann-Dirichlet  $\partial_t\Psi(s,0)=0$ and $\Psi(s,1)=0$ $(s<0)$ for $\mathcal{L}_j$,
\item Neumann-Dirichlet  $\partial_t\Phi(\sigma,0)=0$ and $\Psi(\sigma,1)=0$ $(\sigma<0)$ for $\mathcal{N}^\lef_{j}$,
\item Pure Dirichlet  $\Phi(\sigma,0)=0$ and $\Psi(\sigma,1)=0$ $(\sigma>0)$ for $\mathcal{N}^\ri_{j}$.
\end{enumerate}
Note that
\begin{equation}
\label{E:N0}
   \mathcal{N}^\lef_0 = -\partial^2_\sigma - \frac{1}{2\pi^2}\partial^2_t \quad\mbox{and}\quad
   \mathcal{N}^\ri_0 = -\partial^2_\sigma - \frac{1}{2\pi^2}\partial^2_\tau\,.
\end{equation}
\end{notation}


\subsection{Dirichlet-to-Neumann operators}
Here we introduce the Dirichlet-to-Neumann operators $T^{\ri}$ and $T^{\lef}$ which we use to solve the problems in the variables $(\sigma,t)$. We denote by $I$ the interface $\{0\}\times(0,1)$ between $\Stri$ and $\Stlef$.

On the right, and with Notation \ref{6not}, we consider the problem:
\[
   \left(\mathcal{N}^\ri_{0}-\frac{1}{8}\right)\Phi_\ri=0\ \ \mbox{in}\ \ \Stri
   \quad \mbox{and}\quad  \Phi_\ri(0,t)=G(t)
\]
where  $G\in H_{00}^{1/2}(I)$. Since the first eigenvalue of the transverse part of $\mathcal{N}^\ri_{0}-\frac{1}{8}$ is positive, this problem has a unique exponentially decreasing solution $\Phi_\ri$. Its exterior normal derivative $-\dr_{\sigma}\Phi_{\ri}$ on the line $I$ is well defined in $H^{-1/2}(I)$. \Bk We define:
\[T^{\ri}G=\dr_{n}\Phi_{\ri}=-\dr_{\sigma}\Phi_{\ri}\,.\]
We have
\[\langle T^\ri G,G\rangle=Q_{\ri}(\Phi_{\ri})\geq C\|G\|^2_{\sH^{1/2}_{00}(I)}\,.\]
On the left, we consider the problem:
\[
   \Big(\mathcal{N}^\lef_{0}-\frac{1}{8} \Big)\Phi_\lef=0\ \ \mbox{in}\ \ \Stlef
   \quad \mbox{and}\quad  \Phi_\lef(0,t)=G(t)
\]
where $G\in \sH^{1/2}_{00}(I)$.

For all $G\in \sH_{00}^{1/2}(I)$ such that $\Pi_0G=0$ (where $\Pi_{0}$ is defined in \eqref{Pi0}), this problem has a unique exponentially decreasing solution $\Phi_\lef$. Its exterior normal derivative $\dr_{\sigma}\Phi_{\lef}$ on the line $I$ is well defined in $\sH^{-1/2}(I)$. We define:
$$T^{\lef}G=\dr_{n}\Phi_{\lef}=\dr_{\sigma}\Phi_{\lef}\,.$$
We have:
$$\langle T^\lef G,G\rangle=Q_{\lef}(\Phi_{\lef})\geq 0\,.$$

\begin{prop}
\label{6prop} 
The operator $T^\ri +T^\lef\Pi_{1}$ is coercive on $H^{1/2}_{00}(I)$ with $\Pi_{1}=\Id-\Pi_{0}$. In particular, it is invertible from $\sH^{1/2}_{00}(I)$ onto $\sH^{-1/2}(I)$.
\end{prop}
This proposition allows to prove the following lemma which is in the same spirit as Lemma \ref{lem-N0}, but now for transmission problems on $\Stlef\cup\Stri$ (we recall that $c_0(t) = \cos(\frac\pi2t)$):

\begin{lem}\label{lem-N0lefri}
Let $F_\lef=F_\lef(\sigma,t)$ and $F_\ri=F_\ri(\sigma,\tau)$ be real functions defined on $\Stlef$ and $\Stri$, respectively, with exponential decay with respect to $\sigma$. Let $G^0\in \sH^{1/2}_{00}(I)$ and $H\in \sH^{-1/2}(I)$ be data on the interface $I=\partial\Stlef\cap\partial\Stri$. 
Then there exists a unique coefficient $\zeta\in\R$ and a unique trace $G\in \sH^{1/2}_{00}(I)$ such that the transmission problem
\[
\begin{cases}
   \big(\mathcal{N}^\lef_{0}-\frac{1}{8}\big)\Phi_\lef=F_\lef\quad\mbox{in}\ \ \Stlef,\quad  
   &\Phi_\lef(0,t)=G(t)+G^0(t)+\zeta c_{0}(t)\,, \\
   \big(\mathcal{N}^\ri_{0}-\frac{1}{8}\big)\Phi_\ri=F_\ri\quad\mbox{in}\ \ \Stri,\quad  
   &\Phi_\ri(0,t)=G(t)\,, \\[0.5ex]
   \partial_\sigma\Phi_\lef(0,t)-\partial_\sigma\Phi_\ri(0,t) = H(t)
   \quad\mbox{on}\ \  I,
\end{cases}
\]
admits a (unique) solution $(\Phi_\lef,\Phi_\ri)$ with exponential decay.
\end{lem}

\begin{proof}
Let $(\Phi_{\lef}^0,\zeta_0)$ be the solution provided by Lemma \ref{lem-N0} for the data $F=F_\lef$ and $G=0$. Let $\Phi_{\ri}^0$ be the unique exponentially decreasing solution of the problem
\[
   \Big(\mathcal{N}^\ri_{0}-\frac{1}{8} \Big)\Phi^0_{\ri}=F_\ri\quad\mbox{in}\quad\Stri,\quad  
   \Phi^0_\ri(0,t)=0\,.
\]
Let $H^0$ be the jump $\partial_\sigma\Phi_{\ri}^0(0,t)-\partial_\sigma\Phi_{\lef}^0(0,t)$. If we define the new unknowns $\Phi_{\ri}^1=\Phi_{\ri}-\Phi_{\ri}^0$ and $\Phi_{\lef}^1=\Phi_{\lef}-\Phi_{\lef}^0$, the problem we want to solve becomes
\begin{align*}
   \Big(\mathcal{N}^\lef_{0}-\frac{1}{8} \Big)\Phi_{\lef}^1&=0\quad\mbox{in}\quad\Stlef,\quad  
   \Phi_{\lef}^1(0,t)=G(t)+(\zeta-\zeta_0) c_{0}(t)\,, \\
   \Big(\mathcal{N}^\ri_{0}-\frac{1}{8} \Big)\Phi_{\ri}^1&=0\quad\mbox{in}\quad\Stri,\quad  
   \Phi_{\ri}^1(0,t)=G(t)\,, \\
   \partial_\sigma\Phi_{\ri}^1(0,t)-\partial_\sigma\Phi_{\lef}^1(0,t) &= H(t)-H^0(t)
   \quad\mbox{on}\quad I\,.
\end{align*}
Using Proposition \ref{6prop} we can set $G=(T^\ri +T^\lef\Pi_{1})^{-1}(H-H_0)$, which ensures the solvability of the above problem. 
\end{proof}


\subsection{Construction of quasimodes}
\label{S:512}
\subsubsection{Terms of order $h^0$}
Let us write the ``interior" equations:
\begin{align*}
\lef_{s} &:&\mathcal{L}_{0}\Psi_{\lef,0}&=\gamma_{0}\Psi_{\lef,0}\\ 
\lef_{\sigma} &:&\mathcal{N}^\lef_{0}\Phi_{\lef,0}&=\gamma_{0}\Phi_{\lef,0}\\
\ri\ &:&\mathcal{N}^\ri_{0}\Phi_{\ri,0}&=\gamma_{0}\Phi_{\ri,0}\,.\hskip5em
\end{align*}
The boundary conditions are:
$$\Psi_{\lef,0}(0,t)+\Phi_{\lef,0}(0,t)=\Phi_{\ri,0}(0,t)\,,$$
$$ \dr_{\sigma}\Phi_{\lef,0}(0,t)=\dr_{\sigma}\Phi_{\ri,0}(0,t)\,.$$
We get:
$$\gamma_{0}=\frac{1}{8},\quad \Psi_{\lef,0}=g_{0}(s)c_{0}(t)\,.$$
We now apply Lemma \ref{lem-N0lefri} with $F_{\lef}=0$, $F_{\ri}=0$, $G_{0}=0$, $H=0$ to get 
$$G=0 \quad\mbox{and}\quad \zeta=0\,.$$
We deduce: $\Phi_{\lef,0}=0$, $\Phi_{\ri,0}=0$ and, since $\zeta=-g_{0}(0)$, $g_{0}(0)=0$. 
At this step, we do not have determined $g_{0}$ yet.

 

\subsubsection{Terms of order $h^{1/3}$}
The interior equations read:
\begin{align*}
\lef_{s} &:&\mathcal{L}_{0}\Psi_{\lef,1}&=\gamma_{0}\Psi_{\lef,1}+\gamma_{1}\Psi_{\lef,0}\\ 
\lef_{\sigma} &:&\mathcal{N}^{\lef}_{0}\Phi_{\lef,1}&=\gamma_{0}\Phi_{\lef,1}+\gamma_{1}\Phi_{\lef,0}\\
\ri &:&\mathcal{N}^{\ri}_{0}\Phi_{\ri,1}&=\gamma_{0}\Phi_{\ri,1}+\gamma_{1}\Phi_{\ri,0}.\hskip5em
\end{align*}
Using Lemma \ref{lem-L00}, the first equation implies:
$$\gamma_{1}=0,\quad \Psi_{\lef,1}(s,t)=g_{1}(s)c_{0}(t)\,.$$
The boundary conditions are:
$$g_{1}(0)c_{0}(t)+\Phi_{\lef,1}(0,t)=\Phi_{\ri,1}(0,t)\,,$$
$$g_{0}'(0)c_{0}(t)+\dr_{\sigma}\Phi_{\lef,1}(0,t)=\dr_{\sigma}\Phi_{\ri,1}(0,t)\,.$$
The system becomes:
\begin{align*}
\lef_{\sigma} &:& \Big(\mathcal{N}_{0}^{\lef}-\frac{1}{8} \Big)\Phi_{\lef,1}&=0,\\
\ri\ &:& \Big(\mathcal{N}_{0}^{\ri}-\frac{1}{8} \Big)\Phi_{\ri,1}&=0.\hskip5em
\end{align*}
We apply Lemma \ref{lem-N0lefri} with $F_{\lef}=0$, $F_{\ri}=0$, $G_{0}=0$, $H=-g_{0}'(0)c_{0}(t)$ to get:
$$G=-g_{0}'(0)(T^\ri +T^\lef\Pi_{1})^{-1}c_{0}\,.$$
Since $G=\Phi_{\ri,1}$ and $\zeta=-g_{1}(0)$, this determines $\Phi_{\lef,1}$, $\Phi_{\ri,1}$ and $g_{1}(0)$. 

\subsubsection{Terms of order $h^{2/3}$}
The interior equations write:
\begin{align*}
\lef_{s}&:&\mathcal{L}_{2}\Psi_{\lef,0}+\mathcal{L}_{0}\Psi_{\lef,2}&=\sum_{l+k=2}\gamma_{l}\Psi_{\lef,k}\\
\lef_{\sigma}&:&\mathcal{N}_{0}^{\lef}\Phi_{\lef,2}&=\sum_{l+k=2}\gamma_{l}\Phi_{\lef,k}\\
\ri&:&\mathcal{N}_{0}^{\ri}\Phi_{\ri,2}&=\frac{1}{8}\Phi_{\ri,2},\hskip5em
\end{align*}
with 
$$\mathcal{L}_{2}\Psi_{\lef,0}=-g_{0}''(s)c_{0}(t)+\frac{1}{\pi^3\sqrt{2}} sg_{0}(s)\dr_{t}^2(c_{0})\,.$$
Lemma \ref{lem-L00} and then Lemma \ref{lem-Ai} imply:
\begin{equation}
\label{E:g0}
   -g_{0}''-\frac{1}{4\pi\sqrt{2}} sg_{0}=\gamma_{2}g_{0}.
\end{equation}
Thus, $\gamma_{2}$ is one of the eigenvalues of the Airy operator  and $g_{0}$ an associated eigenfunction.
In particular, this determines the unknown functions of the previous steps. We are led to take:
$$\Psi_{\lef,2}(s,t)=\Psi_{\lef,2}^{\perp}+g_{2}(s)c_{0}(t), \mbox{ with }\Psi_{\lef,2}^{\perp}=0$$
and to the system:
\begin{align*}
\lef_{\sigma}&:&\Big(\mathcal{N}_{0}^{\lef}-\frac{1}{8} \Big)\Phi_{\lef,2}&=0\\
\ri&:& \Big(\mathcal{N}_{0}^{\ri}-\frac{1}{8} \Big)\Phi_{\ri,2}&=0\,.\hskip5em
\end{align*}
Using Lemma \ref{lem-N0lefri}, we find 
$$G=-g_{1}'(0)(T^\ri +T^\lef\Pi_{1})^{-1}c_{0}\,.$$
This determines $\Phi_{\ri,2}$,  $\Phi_{\lef,2}$ and $g_{2}(0)$. The function $g_{1}$ is still unknown at this step.

This construction can be continued at any order. Up to the addition of a small correction term (to satisfy the transmission condition and to insure that the Ansatz belongs to the domain of the operator), we may apply the spectral theorem, as usual. If we are just interested in the two terms asymptotic expansion, we may just apply the min-max principle (that needs less regularity) with $g_{1}=g_{2}=0$.












==> chapter-vanishing-mod.tex <==
\chapter{Models for vanishing magnetic fields}\label{chapter-vanishing-mod}

\begin{flushright}
\begin{minipage}{0.6\textwidth}
L'explication que nous devons juger satisfaisante est celle qui adh\`ere \`a son objet : point de vide entre eux, pas d'interstice o\`u une autre explication puisse aussi bien se loger ; elle ne convient qu'\`a lui, il ne se pr\^ete qu'\`a elle.
%Sie begriffen, dass die Vernunft nur das einsieht, was sie selbst nach ihrem Entwurfe hervorbringt, dass sie mit Prinzipien ihrer Urteile nach best\"undigen Gesetzen vorangehen und die Natur n\"otigen m\"usse auf ihre Fragen zu antworten, nicht aber sich von ihr allein gleichsam am Leitbande g\"angeln lassen m\"usse; denn sonst h\"angen zuf\"allige, nach keinem vorher entworfenen Plane gemachte Beobachtungen gar nicht in einem notwendigen Gesetze zusammen, welches doch die Vernunft sucht und bedarf.
\begin{flushright}
%\textit{Kritik der reinen Vernunft}, Vorrede, Kant
\textit{La pens\'ee et le mouvant}, Bergson
\end{flushright}
\vspace*{0.5cm}
\end{minipage}
\end{flushright}



We will see that the properties of  ${\mathcal M}^\Neu_{x,\xi}$ be can used to investigate those of  ${\mathcal M}_{x,\xi}$. Therefore we begin by analyzing the family of operators  ${\mathcal M}^\Neu_{x,\xi}$ and we prove Theorem~\ref{theo-Rp} and apply it to prove Theorem~\ref{theo-R}.


\section{Analysis of $\mathcal{M}^\Neu_{x,\xi}$}
\subsection{Changing the parameters}
To analyze the family of operators $\mathcal{M}^\Neu_{x,\xi}$ depending on parameters $(x,\xi)$, we introduce the new parameters $(x,\eta)$ using a change of variables. 
Let us introduce the following change of parameters: 
$$\mathcal{P}(x,\xi)=(x,\eta)=\left(x,\xi+\frac{x^2}{2}\right)\,.$$
A straight forward computation provides that $\mathcal{P} : \R^2\to\R^2$ is a $\mathcal{C}^\infty$-diffeomorphism such that:
$$|x|+|\xi|\to+\infty\Leftrightarrow |\mathcal{P}(x,\xi)|\to+\infty\,.$$
We have $\mathcal{M}^\Neu_{x,\xi}=\mathcal{N}^\Neu_{x,\eta}$, where:
$$\mathcal{N}^\Neu_{x,\eta}=D_{t}^2+\left(\frac{(t-x)^2}{2}-\eta\right)^2\,,$$
with Neumann condition on $t=0$. Let us denote by $\nu_{1}^\Neu(x,\eta)$ the lowest eigenvalue of $\mathcal{N}^\Neu_{x,\eta}$, so that:
$$\mu^\Neu_{1}(x,\xi)=\nu^\Neu_{1}(x,\eta)=\nu^\Neu_{1}\left(\mathcal{P}(x,\xi)\right)\,.$$
We denote by $\Dom(\mathcal{Q}^\Neu_{x,\eta})$ the form domain of the operator and by 
$\mathcal{Q}^\Neu_{x,\eta}$ the associated quadratic form. 

\subsection{Existence of a minimum for $\mu_{1}^\Neu(x,\xi)$}
To prove Theorem \ref{theo-Rp}, we establish the following result:
\begin{theo}\label{theo-Rp2}
The function $\R\times\R\ni (x,\eta)\mapsto \nu_{1}^\Neu(x,\eta)$ admits a minimum. Moreover we have:
$$\liminf_{|x|+|\eta|\to+\infty}\nu_{1}^\Neu(x,\eta)\geq\nu_{\Mont}>\min_{(x,\eta)\in\R^2}\nu_{1}^\Neu(x,\eta)\,.$$
\end{theo}
To prove this result, we decompose the plane in subdomains and analyze in each part. 

\begin{lem}\label{derivees-parabole}
For all $(x,\eta)\in\R^2$ such that $\eta\geq\frac{x^2}{2}$, we have:
$$-\dr_{x}\nu_{1}^\Neu(x,\eta)+\sqrt{2\eta}\dr_{\eta}\nu_{1}^\Neu(x,\eta)>0\,.$$
Thus there is no critical point in the area $\{\eta\geq\frac{x^2}{2}\}$.
\end{lem}

\begin{proof}
The Feynman-Hellmann formulas provide:
\begin{equation*}
\dr_{x}\nu_{1}^\Neu(x,\eta)=-2\int_{0}^{+\infty} \left(\frac{(t-x)^2}{2}-\eta\right)(t-x)u_{x,\eta}^2(t)\,\dx t,
\end{equation*}
\begin{equation*}
\dr_{\eta}\nu_{1}^\Neu(x,\eta)=-2\int_{0}^{+\infty} \left(\frac{(t-x)^2}{2}-\eta\right)u_{x,\eta}^2(t)\,\dx t.
\end{equation*}
We infer:
$$-\dr_{x}\nu_{1}^\Neu(x,\eta)+\sqrt{2\eta}\dr_{\eta}\nu_{1}^\Neu(x,\eta)=\int_{0}^{+\infty}(t-x-\sqrt{2\eta})(t-x+\sqrt{2\eta})(t-x-\sqrt{2\eta})u_{x,\eta}^2(t)\,\dx t\,.$$
We have:
$$\int_{0}^{+\infty}(t-x-\sqrt{2\eta})^2(t-x+\sqrt{2\eta})u_{x,\eta}^2(t)\,\dx t>0\,.$$
\end{proof}

\begin{lem}\label{lem.minnuad}
We have:
$$\inf_{(x,\eta)\in\R^2}\nu_{1}^\Neu(x,\eta)<\nu_{\Mont}\,.$$
\end{lem}
\begin{proof}
We apply Lemma \ref{derivees-parabole} at $x=0$ and $\eta=\eta_{\Mont}$ to deduce that:
$$\dr_{x}\nu_{1}^\Neu(0,\eta_\Mont)<0\,.$$
\end{proof}

The following lemma is obvious:
\begin{lem}\label{lem.deltaneg}
For all $\eta\leq 0$, we have:
$$\nu_{1}^\Neu(x,\eta)\geq \eta^2\,.$$
In particular, we have
$$\nu_{1}^\Neu(x,\eta)> \nu_{\Mont},\qquad \forall \eta<-\sqrt{\nu_{\Mont}}\,.$$
\end{lem}

\begin{lem}\label{lem.parab}
For $x\leq 0$ and $\eta\leq\frac{x^2}{2}$, we have:
$$\nu_{1}^\Neu(x,\eta)\geq\nu_{1}^{[1]}({0}) >\nu_{\Mont}\,.$$
\end{lem}
\begin{proof}
We have, for all $\psi\in\Dom(\mathcal{Q}^\Neu_{x,\eta})$:
$$\mathcal{Q}^\Neu_{x,\eta}(\psi)=\int_{\R_{+}} |D_{t}\psi|^2+\left(\frac{(t-x)^2}{2}-\eta\right)^2|\psi|^2\dx t$$
and
$$\left(\frac{(t-x)^2}{2}-\eta\right)^2=\left(\frac{t^2}{2}-x t+\frac{x^2}{2}-\eta\right)^2\geq \frac{t^4}{4}\,.$$
The min-max principle provides:
$$\nu_{1}^\Neu(x,\eta)\geq\nu_{1}^{[1]}({0})\,.$$
Moreover, thanks to the Feynman-Hellmann theorem, we get:
$$\left(\dr_{\eta}\nu_{1}^{[1]}({\eta})\right)_{\eta=0}=-\int_{\R_{+}}t^2u_{0}(t)^2\dx t<0\,.$$
\end{proof}
\begin{lem}\label{lem.3.6}
There exist $C,D>0$ such that for all $x\in\R$ and $\eta\geq D$ such that $\frac{x}{\sqrt{\eta}}\geq -1$:
$$\nu_{1}^\Neu(x,\eta)\geq C\eta^{1/2}\,.$$
\end{lem}

\begin{proof}
For $x\in\R$ and $\eta>0$, we can perform the change of variable:
$$\tau=\frac{t-x}{\sqrt{\eta}}\,.$$ 
The operator $\eta^{-2}\mathcal{N}^\Neu_{x,\eta}$ is unitarily equivalent to:
$$\hat{\mathcal{N}}^\Neu_{\hat{x},h}=h^2D_{\tau}^2+\left(\frac{\tau^2}{2}-1\right)^2\,,$$
on $\sL^2\left((-\hat{x},+\infty)\right)$, with $\hat{x}=\frac{x}{\sqrt{\eta}}$ and $h=\eta^{-3/2}$. 
With Lemma \ref{lem.3.6-prep}, we infer, using the min-max principle:
$$\nu_{1}^\Neu(x,\eta) \geq c\eta^{-3/2}\,,$$
for $\eta$ large enough.
\end{proof}


\begin{lem}\label{Agmon-Mont}
Let $u_{\eta}$ be an eigenfunction associated with the first eigenvalue of ${\mathfrak L}_{\eta}^{\Mont,+}$. 
Let $D>0$. There exist $\eps_{0},C>0$ such that, for all $\eta$ such that $|\eta|\leq D$, we have:
$$\int_{0}^{+\infty} e^{2\eps_{0} t^3}|u_{\eta}|^2\dx t\leq C\|u_{\eta}\|^2\,.$$
\end{lem}

\begin{proof}
We let $\Phi_{m}=\eps\chi_{m}(t) t^3$. The Agmon estimate provides:
$$\int_{0}^\infty \left(\frac{t^2}{2}-\eta\right)^2|e^{\Phi_{m}} u_{\eta}|^2\dx t\leq \nu_{1}^{[1]}(\eta)
\|e^{\Phi_{m}} u_{\eta}\|^2+\|\nabla\Phi_{m} e^{\Phi_{m}} u_{\eta}\|^2\,.$$
It follows that:
$$\int_{0}^\infty \frac{t^4}{8}|e^{\Phi_{m}} u_{\eta}|^2\dx t\leq (\nu_{1}^{[1]}(\eta)+2\eta^2)\|e^{\Phi_{m}} u_{\eta}\|^2+\|\nabla\Phi_{m} e^{\Phi_{m}} u_{\eta}\|^2\,.$$
We infer that:
$$\int_{0}^\infty t^4|e^{\Phi_{m}} u_{\eta}|^2\dx t\leq M(D)\|e^{\Phi_{m}} u_{\eta}\|^2+8\|\nabla\Phi_{m} e^{\Phi_{m}} u_{\eta}\|^2\,.$$
With our choice of $\Phi_{m}$, we have
$$|\nabla\Phi_{m}|^2\leq 18\eps^2\chi^2_{m}(t)t^4+2\eps^2\chi_{m}'(t)^2 t^6\leq 18\eps^2 t^4+2\eps^2\chi_{m}'(t)^2 t^6\leq  C\eps^2 t^4\,,$$
since $\chi_{m}'(t)^2 t^2$ is bounded. For $\eps$ fixed small enough, we deduce
$$\int_{0}^\infty  t^4|e^{\Phi_{m}} u_{\eta}|^2\dx t\leq \frac{M(D)}{1-8C \eps^2}\|e^{\Phi_{m}} u_{\eta}\|^2
\leq \tilde M(D) \|e^{\Phi_{m}} u_{\eta}\|^2\,.$$
Let us choose $R>0$ such that: $R^4-M(D)>0$. We have:
$$(R^4-\tilde M(D))\int_{R}^{+\infty} e^{2\Phi_{m}}|u_{\eta}|^2\dx t\leq \tilde M(D)\int_{0}^R e^{2\Phi_{m}}|u_{\eta}|^2\,dy\leq \tilde M(D)C(R)\|u_{\eta}\|^2\,,$$
and:
$$\int_{R}^{+\infty} e^{2\Phi_{m}}|u_{\eta}|^2\dx t\leq C(R,D)\|u_{\eta}\|^2\,.$$
We infer:
$$\int_{0}^{+\infty} e^{2\Phi_{m}}|u_{\eta}|^2\dx t\leq \tilde C(R,D)\|u_{\eta}\|^2\,.$$
It remains to take the limit $m\to+\infty$.
\end{proof}


\begin{lem}\label{lem.3.8}
For all $D>0$, there exist $A>0$ and $C>0$ such that for all $|\eta|\leq D$ and $x\geq A$, we have:
$$\left|\nu_{1}(x,\eta)-\nu_{1}^{[1]}({\eta})\right|\leq Cx^{-2}\,.$$
\end{lem}

\begin{proof}
We perform the translation $\tau=t-x$, so that $\mathcal{N}^\Neu_{x,\eta}$ is unitarily equivalent to:
$$\tilde{\mathcal{N}}^\Neu_{x,\eta}=D_{\tau}^2+\left(\frac{\tau^2}{2}-\eta\right)^2\,,$$
on $\sL^2(-x,+\infty)$. The corresponding quadratic form writes:
$$\tilde{\mathcal{Q}}^\Neu_{x,\eta}(\psi)=\int_{-x}^{+\infty} |D_{\tau}\psi|^2+\left(\frac{\tau^2}{2}-\eta\right)^2|\psi|^2\,\dx\tau\,.$$

Let us first prove the upper bound.
We take $\psi(\tau)=\chi_{0}(x^{-1}\tau)u_{\eta}(\tau)$. The \enquote{IMS} formula provides:
$$\tilde{\mathcal{Q}}^\Neu_{x,\eta}(\chi_{0}(x^{-1}\tau)u_{\eta}(\tau))=\nu_{1}^{[1]}({\eta})\|\chi_{0}(x^{-1}\tau)u_{\eta}(\tau)\|^2+\|(\chi_{0}(x^{-1}\tau))'u_{\eta}(\tau)\|^2\,.$$
Jointly min-max principle with Lemma \ref{Agmon-Mont}, we infer that:
\begin{eqnarray*}
\nu_{1}(x,\eta)
&\leq& \nu_{1}^{[1]}({\eta})+\frac{\|(\chi_{0}(x^{-1}\tau))'u_{\eta}(\tau)\|^2}{\|\chi_{0}(x^{-1}\tau)u_{\eta}(\tau)\|^2}\\
&\leq& \nu_{1}^{[1]}({\eta})+\frac{Cx^{-2}}{ e^{2c\eps_{0} x^3}}. 
\end{eqnarray*}
Let us now prove the lower bound.
Let us now prove the converse inequality. We denote by $\tilde{u}_{x,\eta}$ the positive and $\sL^2$-normalized groundstate of $\tilde{\mathcal{N}}^\Neu_{x,\eta}$. On the one hand, with the \enquote{IMS} formula, we have:
$$\tilde{\mathcal{Q}}^\Neu_{x,\eta}(\chi_{0}(x^{-1}\tau)\tilde{u}_{x,\eta})\leq\nu_{1}(x,\eta)\|\chi_{0}(x^{-1}\tau)\tilde{u}_{x,\eta}\|^2+Cx^{-2}\,.$$
On the other hand, we notice that:
$$\int_{-x}^{+\infty} t^4|\tilde{u}_{x,\eta}|^2\,\dx \tau\leq C,\qquad
\int_{-x}^{-\frac{x}{2}} t^4|\tilde{u}_{x,\eta}|^2\,\dx \tau\leq C\,,$$
and thus:
$$\int_{-x}^{-\frac{x}{2}} |\tilde{u}_{x,\eta}|^2\,\dx \tau\leq \tilde Cx^{-4}\,.$$
We infer that:
$$\tilde{\mathcal{Q}}^\Neu_{x,\eta}(\chi_{0}(x^{-1}\tau)\tilde{u}_{x,\eta})\leq (\nu_{1}(x,\eta)+Cx^{-2})\|\chi_{0}(x^{-1}\tau)\tilde{u}_{x,\eta}\|^2\,.$$
We deduce that:
$$\nu_{1}^{[1]}({\eta})\leq \nu_{1}(x,\eta)+Cx^{-2}\,.$$
\end{proof}


We have proved in Lemmas~\ref{lem.deltaneg}-\ref{lem.3.6} and \ref{lem.3.8} that the  limit inferior of $\nu_{1}(x,\eta)$ in these areas are not less than $\nu_{\Mont}$.
Then, we deduce the existence of a minimum with Lemma~\ref{lem.minnuad}.





\section{Analysis of $\mathcal{M}_{x,\xi}$}
Theorem~\ref{theo-R} is a consequence of the following two lemmas.
\begin{lem}
We have:
$$\underline\mu_{1}<\nu_{\Mont}\,.$$
\end{lem}
\begin{proof}
We have 
$$\underline\mu_{1}=\inf_{(x,\xi)\in\R^2}\mu_{1}(x,\xi)\leq \inf_{x\in\R}\mu_{1}(x,0)\,.$$
We use a finite element method, with the Finite Element Library {\sc M\'elina} (see \cite{Melina}), on $[-10,10]$ with Dirichlet condition on the artificial boundary, with 1000 elements $\mathbb P_{2}$. The discretization space for the finite element method is included in the form domain of the operator and thus the computed eigenvalue provides a rigorous upper-bound (see \cite[Section 2]{BDMV07} and \cite[Section 5.1]{BDPR11}).
For any $x$, these computations give a upper-bound of $\mu_{1}(x,0)$.
Numerical computations and Proposition~\ref{conjecture-mont} give
$$\inf_{x\in\R}\mu_{1}(x,0)\leq 0.33227<0.5<\nu_{\Mont}\,,$$
In fact, numerical simulations suggest that $\inf_{x\in\R}\mu_{1}(x,0)\simeq 0.33227$ which is an approximation of the first eigenvalue for $x=0.827$.
\end{proof}


\begin{lem}
For all $(x,\xi)\in\R^2$, we have:
$$\mu_{1}(x,\xi)\geq\min(\mu_{1}^\Neu(x,\xi),\mu_{1}^\Neu(x,-\xi))\,.$$
\end{lem}
\begin{proof}
Let $u$ be a normalized eigenfunction associated with $\mu_{1}(x,\xi)$. We can split:
\begin{eqnarray*}
\mu_{1}(x,\xi)&=&\int_{-\infty}^0|D_{t}u|^2+\left(\frac{t^2}2-x t-\xi\right)^2|u|^2\dx t+\int_0^{+\infty}|D_{t}u|^2+\left(\frac{t^2}2-x t-\xi\right)^2|u|^2\dx t\\
&\geq& \mu_{1}^\Neu(x,-\xi)\int_{-\infty}^0|u|^2\dx t+\mu_{1}^\Neu(x,\xi)\int_0^{\infty}|u|^2\dx t\\
&\geq& \min(\mu_{1}^\Neu(x,-\xi),\mu_{1}^\Neu(x,\xi)).
\end{eqnarray*}
\end{proof}



